Inversion-Free Video Style Transfer with Trajectory Reset Attention Control and Content-Style Bridging

Video style transfer aims to alter the style of a video while preserving its content. Previous methods often struggle with content leakage and style misalignment, particularly when using image-driven approaches that aim to transfer precise styles. In this work, we introduce Trajectory Reset Attention Control (TRAC), a novel method that allows for high-quality style transfer while preserving content integrity. TRAC operates by resetting the denoising trajectory and enforcing attention control, thus enhancing content consistency while significantly reducing the computational costs against inversion-based methods. Additionally, a concept termed Style Medium is introduced to bridge the gap between content and style, enabling a more precise and harmonious transfer of stylistic elements. Building upon these concepts, we present a tuning-free framework that offers a stable, flexible, and efficient solution for both image and video style transfer. Experimental results demonstrate that our proposed framework accommodates a wide range of stylized outputs, from precise content preservation to the production of visually striking results with vibrant and expressive styles.

==> sec/Image_style_transfer.tex <==
\section{Image Style Transfer}
\subsection{Evaluation Protocol}
For quantitative comparison, we employ a recently proposed metric, ArtFID \cite{ArtFID} which evaluates overall style transfer performances with consideration of both content and style preservation and also is known as strongly coinciding with human judgment. Specifically, ArtFID is computed as $ArtFID = (1 + LPIPS) · (1 + FID)$. LPIPS measures content fidelity between the stylized image and the corresponding content image, while FID assesses the style fidelity between the stylized image and the corresponding style image.

\textbf{Dataset.} Our evaluations employ content images from MSCOCO \cite{coco} dataset and style images from WikiArt \cite{wikiart} dataset. All input images are center-cropped to 512 × 512 resolution. , We randomly selected 20 content and 40 style images from each dataset, yielding 800 stylized images as some previous like \cite{StyTR2} have done.

% \subsection{Qualitative Results}
% Fig.x demonstrates the superior style transfer results achieved by our method across a variety of subjects, highlighting its robustness and versatility in adapting to diverse content and styles. The results reveal that our method not only facilitates straightforward color transfer but also effectively captures distinctive features from the style image, such as brush strokes and textures, while also adjusting the background scene to best match the style. This results in visually appealing and dynamic style transfer effects.

%\subsection{Comparison with State-of-the-Art methods}




\textbf{Quantitative Comparison}
We evaluate our proposed method through comparison with
current state-of-the-art methods, including CAST \cite{}, StyTR2\cite{}, DiffuseIT\cite{}, InST \cite{}, StyleID \cite{}, which have a style image as input. 
TODO

\textbf{Qualitative Comparison}
Fig. X presents a visual comparison between our method and other state-of-the-art approaches. Overall, our method achieves the optimal visual balance between enhancing stylistic effects and preserving the original content, while effectively preventing content leakage from the style image. Several key observations can be made from this figure:
First, our methods that do not incorporate inversion or introduce a style medium exhibit significant limitations in content preservation, especially in background details.
Second, although inversion-based methods such as StyleID, InST, and InstantStyle+ demonstrate some ability to preserve content, they fail to fully decouple style and content information, which results in visible content leakage in some synthesized images.
% especially in the fourth row of Fig. 7. If users interpret the waves in the fourth row as part of the style, we show in Sec. 5.5 that content leakage can be controlled by adjusting the negative guidance scale ωi, allowing users to customize the result according to their preferences.

\begin{table}
\centering
\small
\begin{tabular}{c c c c c c}
\hline
Metric & Ours  &  CAST & StyTR$^2$  & DiffuseIT & InST \\ 
\hline
\hline
 $\downarrow$ ArtFID & 37.782 &  34.685 & 30.720 & 40.721 & 40.633 \\ 
 $\downarrow$ FID & 24.457 & 20.395 & 18.890 & 23.065 &  21.571\\ 
 $\downarrow$ LPIPS & 0.484  & 0.6212  & 0.5445 & 0.6921  & 0.8002  \\ 
 \hline 
 \\
\end{tabular}
%}
\caption{Quantitative comparison against existing image style transfer methods.}
\label{tab: image_metric}
\end{table}


